Learn to Compress (LtC): Efficient Learning-based Streaming Video Analytics

Video analytics are often performed as cloud services in edge settings, mainly to offload computation, and also in situations where the results are not directly consumed at the video sensors. Sending high-quality video data from the edge devices can be expensive both in terms of bandwidth and power use. In order to build a streaming video analytics pipeline that makes efficient use of these resources, it is therefore imperative to reduce the size of the video stream. Traditional video compression algorithms are unaware of the semantics of the video, and can be both inefficient and harmful for the analytics performance. In this paper, we introduce LtC, a collaborative framework between the video source and the analytics server, that efficiently learns to reduce the video streams within an analytics pipeline. Specifically, LtC uses the full-fledged analytics algorithm at the server as a teacher to train a lightweight student neural network, which is then deployed at the video source. The student network is trained to comprehend the semantic significance of various regions within the videos, which is used to differentially preserve the crucial regions in high quality while the remaining regions undergo aggressive compression. Furthermore, LtC also incorporates a novel temporal filtering algorithm based on feature-differencing to omit transmitting frames that do not contribute new information. Overall, LtC is able to use 28-35% less bandwidth and has up to 45% shorter response delay compared to recently published state of the art streaming frameworks while achieving similar analytics performance.

==> sections/advantage.tex <==
\nael{This subsection should be a discussion subsection after you introduce LtC}

\textbf{Multi-feedback-loop based approaches suffer in real-time applications.} The state-of-the-art spatial compression mechanism \cite{du2020server} uses a multi-feedback loop for each frame to figure out the locations and the sizes of object regions. In the initial phase, the camera sends low-quality frames to the server so the DNN can create a list of bounding boxes where objects might reside. The list is sent back to the camera as feedback requesting high-quality patches only for the bounding boxes mentioned in the list. This process is repeated multiple times in subsequent phases until satisfactory accuracy is achieved. The problem with this approach is that the multi-feedback loop is valid for a single frame, and depending on the number of feedback used, the results are delayed proportionally to the network round-trip-time (RTT) and server processing time. Even if just two phases are used, the response delay is essentially doubled. We aim to use a neural network model as feedback that persists through a long stream of video frames and can act in a single phase \textcolor{purple}{the concept of phase is not clear to me}.




\textbf{Profiling-based approaches hinder bandwidth savings.} The state-of-the-art temporal compression \cite{li2020reducto} mechanism profiles one-second segments of videos and map them to the best possible action \textcolor{purple}{what do you mean by action? which action are you talking about?}. Initially, the camera sends high-quality unfiltered frames for a period of time to the server. Besides performing the video analytics tasks, the server profiles video segments and registers them against the optimal action into a hashtable. The hashtable is sent back to the camera as feedback, where subsequent video segments are matched against the hashtable, and the registered action is performed. The profiling mechanism is initiated if a video segment does not match any entries in the hashtable. Effectively, both in the initial phase and any environment changes trigger the profiling mechanism. In the case of streaming video analytics, the scenario is very dynamic, and often the video segment does not match any entries in the hashtable. As a result, the camera halts the compression until the updated hashtable arrives from the server. This is a waste of bandwidth as each profiling period is usually long and needs a bulk of new frames. By leveraging the generalization capabilities of the feedback neural network model, the update mechanism is rarely called and can be finished using only a few new frames.



